Deep Generative Model for Joint Alignment and Word Representation

This work exploits translation data as a source of semantically relevant learning signal for models of word representation. In particular, we exploit equivalence through translation as a form of distributed context and jointly learn how to embed and align with a deep generative model. Our EmbedAlign model embeds words in their complete observed context and learns by marginalisation of latent lexical alignments. Besides, it embeds words as posterior probability densities, rather than point estimates, which allows us to compare words in context using a measure of overlap between distributions (e.g. KL divergence). We investigate our model's performance on a range of lexical semantics tasks achieving competitive results on several standard benchmarks including natural language inference, paraphrasing, and text similarity.

==> architectures.tex <==
\section{\label{sec:arch}Architectures}


\paragraph{Generative model} We have two generative components, namely, a categorical distribution over the vocabulary of \Lx and another over the vocabulary of \Ly. We predict the parameter (event probabilities) of each distribution with an affine transformation of a latent embedding followed by the $\softmax$ nonlinearity to ensure normalisation: %
%
%
\begin{subequations}
\begin{align}
f(z_i; \theta) &= \softmax\left(\mathbf W_\txt{1}  z_i + \mathbf b_\txt{1}\right) \\
g(z_{a_j}; \theta) &= \softmax\left( \mathbf W_\txt{2}  z_{a_j} + \mathbf b_\txt{2} \right)
\end{align}
\end{subequations}
%
%
%
%
where $\mathbf W_\txt{1} \in \mathbb R^{\vx \times \dz}$, $\mathbf b_\txt{1} \in \mathbb R^\vx$,  $\mathbf W_\txt{2} \in \mathbb R^{\vy \times \dz}$, $\mathbf b_\txt{2} \in \mathbb R^\vy$, and $\vx$ ($\vy$) is the size of the vocabulary of \Lx (\Ly).


\paragraph{Inference model} We predict approximate posterior parameters using two independent transformations
\begin{subequations}\label{eq:posterior-params}
\begin{align}
\mathbf u_i      &= \mathbf M_\txt{1}  \mathbf h_i + \mathbf c_\txt{1}  \\
\mathbf s_i &= \softplus(\mathbf M_\txt{2}  \mathbf h_i + \mathbf c_\txt{2}) 
\end{align}
\end{subequations} 
of a shared representation $\mathbf h_i \in \mathbb R^\dx$ of the $i$th word in the \Lx sequence $x_1^m$---where 
$\mathbf M_\txt{1}, \mathbf M_\txt{2} \in \mathbb R^{\dz \times \dx}$ are projection matrices, $\mathbf c_\txt{1}, \mathbf c_\txt{2} \in \mathbb R^\dz$ are bias vectors, and the $\softplus$ nonlinearity ensures that variances are non-negative.
To obtain the deterministic encoding $\mathbf h_1^m$, we employ two different architectures: (1) a bag-of-words (\textsc{BoW}) encoder, where $\mathbf h_i$ is a deterministic projection of $x_i$ onto $\mathbb R^\dx$; and (2) a bidirectional (\textsc{BiRNN}) encoder, where $\mathbf h_i$ is the element-wise sum of the $i$th hidden state of two LSTMs (each processing the input in opposite order). 
We use $128$ units for deterministic embeddings, and $100$ units for LSTMs \citep{HochreiterEtAl1997LSTM} and latent representations (i.e. $\dz=100$).









 

==> extensions.tex <==

\subsection{Extensions}


Note that our generative story does not model global features of the \Lx sentence. 
In an attempt to leverage more out of the data, we extend the model with a normally distributed sentence embedding $S$ which we use as additional information when generating word embeddings $Z_i$ as well as \Lx observations. The generative story becomes:
%
\begin{comment}
We use the latent variable $Z$ to generate both languages $x_1^m$ and $y_1^n$. However,  during the inference process the approximation for each factor $Z$ is only conditioned on $x_1^m$, thus during reconstruction each factor features must to take into account both languages. This can lead to a poor reconstruction of $y_1^n$. Each... We propose an extension to cope with the whole context of $x_1^m$ by adding a sentence level latent variable... Motivation... additional monolingual context information based on the distributional hypothesis.
The addition is a latent variable that represents each \Lx sentence $k \in \{1, \ldots, b\}$. $S$ takes values in $\mathbb R^\ds$

The generative story for the sentence level representation is as follows:
\end{comment}
%
\begin{align*}
S &\sim \mathcal N(\mathbf 0, \mathbf I) \\ %
Z_i|s &\sim \mathcal N(h(s; \theta), \mathbf I) \\ %
X_i|s, z_i &\sim \Cat(f(s, z_i; \theta)) \\ %
A_j|m &\sim \mathcal U(1/m) \\ %
Y_j|z_1^m, a_j &\sim \Cat(g(z_{a_j}; \theta))  %
\end{align*}
%
We make a hierarchical approximation
\begin{equation}
q_\phi(s|x_1^m) \times q_\phi(z_1^m|s, x_1^m, y_1^n)
\end{equation}
where the first factor is a diagonal Gaussian
\begin{equation}
\begin{aligned}
q_\phi(s|x_1^m) \triangleq  \mathcal N(s|\mathbf u_k, \diag(\mathbf s_k))
\end{aligned}
\end{equation}
and the second is an extension of Equation (\ref{eq:qz}) which conditions on $s$
\begin{equation}
\begin{aligned}
q_\phi(z_1^m|s, x_1^m) \triangleq  \prod_{i=1}^m \mathcal N(z_i|\mathbf l_i, \diag(\mathbf r_i))
\end{aligned}
\end{equation}
where $\mathbf l_i \triangleq \mu_i(s, x_1^m; \phi)$ and $\mathbf r_i \triangleq \sigma_i^2(s, x_1^m; \phi)$. In practice, these are MLPs with longer input vectors (the concatenation of $s$ and a representation of $x_i$.

The new latent variable introduces an additional $\KL$ term into the $\ELBO$, namely, $\KL[q(S) || p(S)]$, and replaces $\KL[q(Z)|| p(Z)]$ by $\KL[q(Z|S)|| p(Z|S)]$. While the former can be computed analytically, the latter can only be approximated by conditioning on a sample $s$.

\begin{equation}\label{eq:ELBO_S}
\begin{aligned}
\log P_\theta(x_1^m, y_1^n|m, n) \ge \\ %
 \sum_{i=1}^m \mathbb E \left[ \log P_\theta(x_i|Z_i); \mathbf u_i, \mathbf s_i \right] \\
 + \sum_{j=1}^n \mathbb E \left[  \log \sum_{a_j=1}^m P(a_j|m) P_\theta(y_j|Z_{a_j}); \mathbf u_1^m, \mathbf s_1^m \right] \\
 - \sum_{i=1}^m \KL\left[\mathcal N(\mathbf l_i, \mathbf r_i) || \mathcal N(h(s_k; \theta), \mathbf I)\right] \quad \\ 
 - \sum_{k=1}^b \KL\left[\mathcal N(\mathbf u_k, \mathbf s_k) || \mathcal N(\mathbf 0, \mathbf I)\right] \quad.
\end{aligned}
\end{equation}

\begin{equation}\label{eq:marginal_s}
\begin{aligned}
P_\theta(x_1^m, y_1^n|m, n) = \\  \int \int p(s_1^b) \prod_{k=1}^b \prod_{i=1}^m  p(z_1^m | s_k)  P_\theta(x_i|z_i, s_k) \\
 \times \prod_{j=1}^n \sum_{a_j=1}^m P(a_j|m) P_\theta(y_j|z_{a_j}) \dd z_1^m \dd s_1^b
\end{aligned}
\end{equation}

The second proposed extension for incorporating the distributional hypothesis is based on self attention across the latent variables at word level $Z$. 

\begin{equation}
\begin{aligned}
\prod_{i=1}^m p_\theta(z_i|z_{i-1}, S) \\
\prod_{i=1}^m p_\theta(x_i|z_i, f(Z; \theta)) \\
\prod_{j=1}^m \sum_{aj=1}^n p_\theta(a_j|n) p_\theta(y_j, z_{aj})
\end{aligned}
\end{equation}

where $f(.)$ is the soft attention computed between the word level latent variables and  $x$. 
\begin{subequations}
\begin{align}
f(Z; \theta) &= \sum_{k \neq i}^m \alpha_k z_k 
\end{align}
\end{subequations}



==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU General Public License.
%
% See the files LICENSE_LPPL and LICENSE_GPL for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

\tikzset{>={triangle 45}}

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->,#1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->,#1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}


